Norm-Range Partition: A Universal Catalyst for LSH based Maximum Inner Product Search (MIPS)

Recently, locality sensitive hashing (LSH) was shown to be effective for MIPS and several algorithms including $L_2$-ALSH, Sign-ALSH and Simple-LSH have been proposed. In this paper, we introduce the norm-range partition technique, which partitions the original dataset into sub-datasets containing items with similar 2-norms and builds hash index independently for each sub-dataset. We prove that norm-range partition reduces the query processing complexity for all existing LSH based MIPS algorithms under mild conditions. The key to performance improvement is that norm-range partition allows to use smaller normalization factor most sub-datasets. For efficient query processing, we also formulate a unified framework to rank the buckets from the hash indexes of different sub-datasets. Experiments on real datasets show that norm-range partition significantly reduces the number of probed for LSH based MIPS algorithms when achieving the same recall.

==> experiment-append-bit16.tex <==
\begin{figure*}[t]
	\input{top20-bit16/Cross-LSH}
	\caption{top20-bit16 Precision Recall comparison with Cross-LSH. } 
	\label{top20-bit16:Cross comparision}
\end{figure*}  

\begin{figure*}[t]
	\input{top20-bit16/netflix}
	
	\input{top20-bit16/yahoomusic}
	
	\input{top20-bit16/imagenet}
	
	\caption{top20-bit16 Precision Recall comparison with Norm-Range-LSH. } 
	\label{top20-bit16:Norm-Range comparision}
\end{figure*} 

==> experiment-append-bit64.tex <==
\begin{figure*}[t]
	\input{top20-bit64/Cross-LSH}
	\caption{top20-bit64 Precision Recall comparison with Cross-LSH. } 
	\label{top20-bit64:Cross comparision}
\end{figure*}  

\begin{figure*}[t]
	\input{top20-bit64/netflix}
	
	\input{top20-bit64/yahoomusic}
	
	\input{top20-bit64/imagenet}
	
	\caption{top20-bit64 Precision Recall comparison with Norm-Range-LSH. } 
	\label{top20-bit64:Norm-Range comparision}
\end{figure*} 

==> experiment-append-top1.tex <==
\begin{figure*}[t]
	\input{top1-bit32/Cross-LSH}
	\caption{top1-bit32 Precision Recall comparison with Cross-LSH. } 
	\label{top1-bit32:Cross comparision}
\end{figure*}  

\begin{figure*}[t]
	\input{top1-bit32/netflix}
	
	\input{top1-bit32/yahoomusic}
	
	\input{top1-bit32/imagenet}
	
	\caption{top1-bit32 Precision Recall comparison with Norm-Range-LSH. } 
	\label{top1-bit32:Norm-Range comparision}
\end{figure*}

==> experiment-append-top10.tex <==
\begin{figure*}[t]
	\input{top10-bit32/Cross-LSH}
	\caption{top10-bit32 Precision Recall comparison with Cross-LSH. } 
	\label{top10-bit32:Cross comparision}
\end{figure*}  

\begin{figure*}[t]
	\input{top10-bit32/netflix}
	
	\input{top10-bit32/yahoomusic}
	
	\input{top10-bit32/imagenet}
	
	\caption{top10-bit32 Precision Recall comparison with Norm-Range-LSH. } 
	\label{top10-bit32:Norm-Range comparision}
\end{figure*}

==> experiment-append-top50.tex <==
\begin{figure*}[t]
	\input{top50-bit32/Cross-LSH}
	\caption{top50-bit32 Precision Recall comparison with Cross-LSH. } 
	\label{top50-bit32:Cross comparision}
\end{figure*}  

\begin{figure*}[t]
	\input{top50-bit32/netflix}
	
	\input{top50-bit32/yahoomusic}
	
	\input{top50-bit32/imagenet}
	
	\caption{top50-bit32 Precision Recall comparison with Norm-Range-LSH. } 
	\label{top50-bit32:Norm-Range comparision}
\end{figure*} 
